An Empirical Analysis of SMS Scam Detection Systems

The short message service (SMS) was introduced a generation ago to the mobile phone users. They make up the world's oldest large-scale network, with billions of users and therefore attracts a lot of fraud. Due to the convergence of mobile network with internet, SMS based scams can potentially compromise the security of internet services as well. In this study, we present a new SMS scam dataset consisting of 153,551 SMSes. This dataset that we will release publicly for research purposes represents the largest publicly-available SMS scam dataset. We evaluate and compare the performance achieved by several established machine learning methods on the new dataset, ranging from shallow machine learning approaches to deep neural networks to syntactic and semantic feature models. We then study the existing models from an adversarial viewpoint by assessing its robustness against different level of adversarial manipulation. This perspective consolidates the current state of the art in SMS Spam filtering, highlights the limitations and the opportunities to improve the existing approaches.

==> files/introduction.tex <==
SMS (Short Message Service) has become a popular way of communication all over the world. SMS usage has grown as a result of telecom providers lowering the cost of SMS services. SMS is widely used in financial transactions, such as bank transfers, mobile money, bill payments, and notification of upcoming due dates, as well as Two-factor authentication (2FA) as one-time passwords (OTP). Due to the regularity and familiarity of these SMS communications, attackers occasionally send identical messages as spam or fraud, attempting to obtain private information or swindle recipients by sending funds to a third-party scam via legal traffic.

SMS scams have grown in popularity in recent years. A recent report from the Australian Competition and Consumer Commission (ACCC) ScamWatch\footnote{https://www.scamwatch.gov.au/scam-statistics} shows that scams conducted by phone or text outweigh those done via social media or email. ScamWatch reported a near-doubling of annual losses (AUD 3,091,790) between 2020 and 2021 (AUD 5,889,596). In August, there were 39,531 SMS fraud reports, up from 32,337 last year. Concerns include an increase in cost per event (total reported losses divided by number of incidents), indicating a change in the effect of these frauds. An estimated USD 86 million was lost to SMS scammers in the US last year(reported by Federal Trade Commission reported\footnote{https://www.ftc.gov/}), and the UK Office of Communications\footnote{https://www.ofcom.org.uk/phones-telecoms-and-internet/advice-for-consumers/scams} recorded a substantial spike in scam texts received by UK citizens. According to Proofpoint\footnote{https://www.proofpoint.com/us/blog/threat-protection/mobile-phishing-increases-more-300-2020-chaos-continues}, because of the rising number of people conducting business online, SMS text messaging frauds surged by 328 percent in Q3 2020 compared to the previous quarter. The rise in scams has been especially troubling for individuals and companies whose clients lack appropriate security understanding; scammers are taking advantage of these easy targets.

Unlike email scams, which have excellent spam filters to stop them, telecommunication companies are improving their SMS scam and spam detection skills. SMS scams aren't simply about financial fraud. Many Android users in Australia have recently been targeted with SMS texts containing Android malware capable of obtaining online banking credentials. 

Scammers frequently use real-life circumstances to deceive. The COVID epidemic has prompted individuals to work from home, take time off, or even be laid off, leading to an increase in online purchasing and internet usage. Most harmful efforts target hundreds of phone numbers consecutively (beginning with ``0400 000 000''), randomly (to appear less predictable), or exploiting stolen lists of legitimate numbers. Though most mobile devices offer features to ban or filter numbers, like email spam/scam filters, these methods are only as effective as user complaints. Scammers utilize sophisticated technology to transmit huge amounts of SMS messages quickly, and frequently use spoofed no to seem authentic or to avoid detection by the phone's automated filter or the user.

While telephone fraud have been extensively discussed and analyzed, the SMS spam and scams have received little attention in the academia. Various techniques to combating SMS-based scams have been developed, however scammers' dynamic nature frequently defeats security barriers. Traditional machine learning and deep learning methods have substantially improved spam detection in email filters; however, spam detection in SMS still requires a lot more research. The focus of this paper is to investigate the landscape of fraudulent and spam SMS messages, existing methods for combating SMS scams, state-of-the-art research in SMS spam defense, and to analyse how current tactics may be abused by scammers and subsequently identify the requirements that are crucial to an acceptable solution. There are a no of challenges including non-availability of publicly large datasets of spam SMS, message ambiguity due to short length and more importantly adversarial attacks like paraphrasing and spacing etc of spam keywords in the text messages to bypass spam detection. SMS dataset was collected from various sources over the previous decade for this purpose. This study will assist drive the development of successful SMS spam defenses, as well as providing a framework for evaluating SMS spam methods.

Contributions of the paper are:
\begin{itemize}
\item {\bf Large scale spam Dataset.} We aggregate and characterise publicly available spam dataset. Given that the benchmark dataset \ik{reference} used for SMS SPAM research is outdated and incomplete consisting only 5,471 messages with 13\% SPAM and 87\% non-SPAM (or HAM) messages, it is not suitable for detecting the most recent, stealthy SMS spam even using advanced machine or deep learning techniques. We propose data collection methods to crawl 57,691 SMS messages from spam observatories such as ScamWatch  \ik{reference} and Action Fraud \ik{reference}. We labelled the dataset into Spam and non-Spam messages constituting 17,300 (30\%) and 40,391 (70\%) SMSes, respectively. 
\item {\bf Valuation of machine learning models.} Given the imbalance nature of the SMS spam datasets, we propose one-class learning and positive unlabelled (PU) learning algorithms. We evaluate several machine learning models on our labelled dataset. The PU learning is a semi-supervised binary classification method that recovers labels from unknown cases in the data by learning from the positive cases in the data and applying what it has learned to re-label the unknown cases. This approach provides benefits to any machine learning problem that requires binary classification on unreliable or unknown data, regardless of the domain. \ik{To the best of our knowledge, the notion of PU learning for spam detection or text classification was never explored earlier.} \ik{Verify this.}

We evaluate and compare the performance of PU learning and one-class learning models with both traditional/ classical two class ML as well as with the state of the art neural network and deep learning  such as the latest transformers based architecture \ik{reference please}.
Additionally, we analyse the aforementioned models with different set of features/ word
embeddings (keeping the pros and cons of each in mind) starting from Non-semantic
Count based Vector space model (Count Vectorization, Tf-IDF) to semantic Non
Context-Based Vector Space Model (Word2Vec by Google, FastText by Facebook,
Glove by Stanford) with static and dynamic modes and finally with semantic ContextBased Vector Space Models (BERT, ELMo etc).

\item {\bf Adversarial machine learning.} To evade detection, spammers may leverage obfuscation or perturbation methods \ik{reference} to Smish\footnote{Smishing is one such SMS spam campaign, where the scammers send a compelling text message to trick targeted recipients into clicking a link and sending the attacker private information or downloading malicious programs to a smartphone}\ik{reference} or Punnycode \ik{reference} spam SMS texts and embedded URLs. We evaluate the robustness of machine learning models against 4 types of adversarial perturbations: charlevel, word-level, sentence-level, and multi-level attacks. To the best of our knowledge, such extensive adversarial
assessment of the ML/DL models have not been performed before.
% \item Performance of One class ML models and their robustness against blackbox attacks and their robustness against blackbox attacks 
% \item Performance of PU ML models and their robustness against blackbox attacks
% \item Performance of conventional ML models and their robustness against blackbox attacks
% \item A new data set comprising messages from the last decade
\end{itemize}


==> files/methodology.tex <==
\section{Methods / Experimental Setup}
To identify the state-of-the-art in preventing SMS scams, we gathered existing techniques and counter measures from academic, industry, Internet domain, and systematically categorize them. The study was designed and conducted according to the stages illustrated in the Figure 1, which are described next:
\subsection{The Super Spam SMS dataset - A decade of messaging}
The Super SMS Spam corpus is a dataset of labeled SMS messages (communicated over the last decade) that have been collected for spam research from public and free for research sources at the internet. The previously used benchmark SMS spam datasets are extremely outdated. The NUS ~\cite{chen2013creating} and UCI ~\cite{almeida2013towards} ~\cite{hidalgo2012validity} ~\cite{almeida2011contributions} are most widely used for SMS spam research. However, the NUS dataset and the UCI dataset were last updated on March 09, 2015 ~\cite{githubnus} and June 22, 2012 ~\cite{UCIMLRep} respectively. Since the threat landscape has significantly evolved over the last couple of years due to the exponential increase in online services and ongoing COVID19 pandemic, therefore there is a need for updated dataset covering all the latest scams. 
\subsubsection{Data Collection}
We did a comprehensive survey in order to identify and collect all of the public SMS spam and scam data. Details of different SMS dataset consolidated in the super dataset are given in Table 1. We call it the super dataset, since it is comprise of all the publicly available labelled and unlabeled datasets, and recently reported Spam SMS messages collected online and from different volunteers. The volunteers were made aware that their contributions were going to be made publicly available. All of the SMS messages from the unlabeled dataset and new spam messages that we collected from different volunteers were labelled manually after pre-processing (ref pre-processing subsection). Moreover, a list of 102 spam SMS messages (reported online) were added to the super dataset to cover the known categories of spam SMS ~\cite{scamtypes} and the recent spam trend. Screenshots of recent spam trending SMS messages from the Scamwatch (Australian Competition and Consumer Commission’s website to help people/ users recognize scams and avoid them) and Action Fraud (UK's national reporting centre for fraud and cyber-crime)\footnote{ https://www.actionfraud.police.uk/} were manually extracted and converted to text using OCR tool (https://www.onlineocr.net/ or mention the python tool). Resultantly, we consolidated a corpus of 161,551 SMS instances in different languages from public and free for research sources. 

% \begin{tabular}{*60}    \toprule
% \emph{Feature Model} & \emph{Classifier} & \emph{Recall}&\emph{Precision}& &\emph{Accuracy} \\\midrule
% Models    & A  & B  & C  & D  \\ 
% \rowcolor{blue!50} Model $X$ & X1 & X2 & X3 & X4\\ 
% \rowcolor{green!50} Model $Y$ & Y1 & Y2 & Y3 & Y4\\\bottomrule
%  \hline
% \end{tabular}


% {\rowcolors{3}{green!80!yellow!50}{green!70!yellow!40}
% \begin{tabular}{ |p{3cm}|p{3cm}|p{3cm}|  }
% \hline
% \multicolumn{3}{|c|}{Country List} \\
% \hline
% Country Name or Area Name& ISO ALPHA 2 Code &ISO ALPHA 3 \\
% \hline
% Afghanistan & AF &AFG \\
% Aland Islands & AX   & ALA \\
% Albania &AL & ALB \\
% Algeria    &DZ & DZA \\
% American Samoa & AS & ASM \\
% Andorra & AD & AND   \\
% Angola & AO & AGO \\
% \hline
% \end{tabular}


\begin{table}
\begin{center}
\caption{Characterization of Super Spam SMS Corpus}
\label{tab:dataset}
\def\arraystretch{1.25}%
%\begin{tabular}{|c c c c c|}
\begin{tabular}{|c c c c|} 
 \hline
 {\bf Dataset} & {\bf \# of SMS} & {\bf Language} & {\bf Labeling} \\%& Main Papers/ Source\\ [0.5ex]
 \hline\hline
DS1~\cite{almeida2013towards}~\cite{hidalgo2012validity}~\cite{almeida2011contributions} & 5,574 & English & Labelled 
\\%& UCI~\cite{almeida2013towards}~\cite{hidalgo2012validity}~\cite{almeida2011contributions}\\ 
 \hline
 DS2~\cite{chen2013creating} & 67,063 & English, Chinese & Unlabeled \\%& NUS ~\cite{chen2013creating}\\
 \hline
 DS3~\cite{githubbansalspamdetection} & 77,039 & English, Roman Hindi & Unlabeled \\%& Github ~\cite{githubbansalspamdetection}\\
 \hline
 DS4~\cite{githubnoorulhasansmsspam} & 557 & English & Labelled \\%& Github ~\cite{githubnoorulhasansmsspam}\\
 \hline
 DS5 ~\cite{gupta2018comparative} & 3,318 & English, Roman Hindi & Labelled \\ 
 \hline
  DS6~\cite{githubFiltro} & 8,000 & Portuguese & Labelled \\ %[1ex] 
 \hline
   DS7\ik{Cite, Volunteers} & 241 & English & Labelled   \\ %[1ex] 
 \hline
    DS8 \ik{Cite, Scamwatch, ActionFraud} & 131 & English & Labelled \\ %[1ex] 
 \hline
 \hline
 Super Dataset \ik{Cite} & \ik{XX} & \ik{LANG} & \ik{Labelled} \\
 \hline
\end{tabular}
\end{center}
\end{table}

\subsubsection{Pre-processing}
We perform pre-processing of the consolidated to remove any inconsistency in the data and refine the data to a form that is suitable for subsequent analysis. For this purpose, we filter out SMS messages in non-english languages, remove duplication and then labelled all of the unlabeled instances in the dataset. We employed a two pass filtering mechanism in order to filter the large amount of non-english SMS messages from the consolidated dataset. In the first pass, we use langdetect (an open source python library for language detection) ~\cite{ langdetecturl} to determine the language of each SMS and filter out SMS in non-english languages. We then passed the filtered SMS messages returned by langdetect to Googletrans (Google API for language detection and translation) ~\cite{googlelangurl} to further filter out the non-english SMS messages. The Googletrans API was kept in the second time due to the limitation of API calls for free user and time consumption in getting the response of each SMS instances since the Googletrans API is a cloud base service as opposed to the langdetect python library which is installed and kept locally. In order to remove the duplicate SMS messages, we imported the SMS corpus in mysql table and deleted the duplicate rows. Finally, we manually labelled all of the remaining unlabeled SMS messages (more than 50,000) as spam and ham (legitimate). After pre-processing, we get a dataset of 57,691 unique SMS messages in English language. Some of the important observations to note here: first, the  dataset is unbalanced, it has a total of 40,391 (70.01 \%) Ham messages and a total of 17,300 (29.99 \%) spam messages. Secondly, the messages are quite short; with an average length of 14.5XXX words, which pose a challenge for content-based filtering algorithms.

% \begin{table}
% \begin{center}
% \caption{Pre-processed Dataset}
% \def\arraystretch{1.25}%
% \begin{tabular}{||c c||}
% \hline
% \multicolumn{2}{|c|}{Total No of SMS Messages After Pre-processing= 57,691} \\
%  \hline\hline
%  Spam messages & 17,300 (29.99 \%) \\ [0.5ex]
%  \hline
%  Ham messages & 40,391 (70.01 \%) \\ [0.5ex]
%  \hline
% \end{tabular}
% \end{center}
% \end{table}

\begin{figure}
\caption{Study Roadmap}
\centering
\includegraphics[width=0.9\textwidth]{img/roadmap.jpg}
\end{figure}

\subsection{Text Pre-processing}
With the help of NLP library NLTK [footnote], we first removed the punctuation and special symbols from the dataset and tokenized each SMS into words. We then lower case all of the SMS messages in the dataset since NLP models are case sensitive. Finally, we removed the Stop words in English from all of the SMS messages.
% \subsection{Dataset Preparation} 
% As discussed in the previous section, we prepared a dataset by collecting spam SMS messages from of public/ free for research sources and recently reported spam SMS messages and performing some pre-processing. We called/ named the resultant dataset, a super dataset since it is composed of most of the SMS scams types and the messages reported over the last decade.
\subsection{Thesaurus creation} We extracted a vocabulary of the 300 most frequent keywords from the spam dataset. A visualization of the most repeated words in the spam messages are shown in Figure 2. 
After processing each SMS, we will create the WordCloud for Spam and Ham messages for the visual representation of widely used words in both Spam and Ham messages.

\begin{figure}
\caption{Top ranked spam keywords}
\centering
\includegraphics[width=0.5\textwidth]{img/cloud1.png}
\end{figure}

\subsection{Document encoding and vectorization} 
We converted the list of words in each message to an actual vector so that the machine learning model can understand it. We generated both syntactic and semantic feature vectors to compare the impact of different feature types on the accuracy of classifiers. All messages in the dataset are encoded using different embedding used in text classification for creating feature from the SMS text. A categorization of the embedding’s used in this study is illustrated in the Figure 3.

\subsubsection{Syntactic / Non-semantic Count based Vector space model}
We applied non-semantic techniques like bag of words (BoW) [ref], n-grams [ref], and TF-IDF [ref] to convert raw text to numerical features. The BoW is a simple method to convert raw text to numerical vectors. BoW model captures the frequencies of the word occurrences in a text corpus. However, the drawback with this model is that it is very sparse, and it does not take into consideration the order of words in which they appear in the document. Therefore, we then applied N-grams, which is a sequence of N-words in a document. Instead of a single word count, we can count the word pairs (bigrams, trigrams etc.). The problem with N-gram is that even here, the resulting matrix is extremely sparse. Finally, we transformed the entire bag-of-words and N-grams corpus into TF-IDF (term frequency-inverse document frequency) corpus each. The TF-IDF feature is an important statistical measure which measures how important a particular word is with respect to a document (SMS) and the entire corpus. Words which are rare in a document will have a high score in the TF-IDF vector. These mappings capture lexical features while ignoring semantics

\subsubsection{Semantic} In order to capture word similarities / semantics and the context in which the words are used together, we created semantic feature vector for each of the following.

\subsubsection{Non Context-Based Vector Space Model}
\begin{description}
\item[Word2Vec[ref]] Word2Vec as the name suggests is a technique that uses a neural network to generate a vector representation for words or tokens and captures semantic similarity between words.
\item[GloVe[ref]] XXXXXXXXXXX
\item[FastText[ref]] Fast Text, an extension of the word2vec model, is another common word embedding method developed by Facebook in 2016. Considered better than word2vec, compute word not present in corpus and also much faster than other methods.

Word2Vec and bag-of-words/tf-idf are somewhat obsolete in 2018 for modeling. For classification tasks, fasttext (https://github.com/facebookresearch/fastText) performs better and faster.
\end{description}

\subsubsection{Context-Based Vector Space Model}
\begin{description}
\item[BERT[ref]] Word2vec provides context-free embeddings (static) whereas BERT gives contextualised embeddings (dynamic). For instance, take these two sentences "I like apples", "I like apple MacBooks". Word2vec will give the same embedding for the word apple in both sentences whereas BERT will give you a different one depending on the context...
\item[ELMo[ref]] XXXXXXXXXX
\end{description}

\begin{figure}
\caption{Word embedding used for encoding/ feature extraction in this study}
\centering
\includegraphics[width=0.8\textwidth]{img/embed.png}
\end{figure}

\subsection{Classification Techniques}
In order to develop/ identify an efficient model for spam detection, we use three machine learning approaches; two-class SVM, one-class SVM and positive and un-labelled (PU) learning.

\subsection{Computing Environment}
All of the algorithm were executed on a server with Linux operating system, 128 Gb RAM, 40 Cores of CPU and 2TB harddrive.

\subsection{Classification and Evaluation}

Performance of existing machine learning classifiers as benchmark in Table 3

Using BERT Encoding to Tackle the Mad-lib Attack in SMS Spam Detection:
https://arxiv.org/abs/2107.06400#

\textbf{Check Performance against paraphrasing/synonym replacement, ham word injection and spam words spacing...}

\subsubsection{Two-class SVM}
We used two-class SVM in our study to discover potential spatial relationships throughout the feature sets. A two-class SVM classifier model using Scikit-learn \footnote{https://scikit-learn.org/} is used using python language in the pycharm environment for this purpose.

\textbf{Model Building and Evaluation} With messages transformed as vectors, we trained the two class SVM algorithm over the TF-IDF corpus by keeping 80/20 ratio (training set is 80\% whereas test size is 20\% of the entire dataset). 
Explain the model parameters SVC(kernel="linear", gamma='scale', random state=3).
We evaluated the model performance on the test data; performance details (Precision, recall and accuracy) of the model is presented in Table 3.

\textbf{Adversarial Evaluation of Model Performances (Evading the Model)} After evaluating the model on unseen test data, we checked the robustness of the model against the adversarial attacks. The adversarial attacks aim to manipulate actions that aim to undermine machine learning performance, cause model misbehavior.

In 2019, Chen and his colleagues at IBM Research, Amazon, and the University of Texas showed that adversarial examples also applied to text classifier machine learning algorithms such as spam filters and sentiment detectors ~\cite{lei2018discrete}. Dubbed ‘paraphrasing attacks’, text-based adversarial attacks involve making changes to sequences of words in a piece of text to cause a misclassification error in the machine learning algorithm.
Like any cyber-attack, the success of adversarial attacks depends on how much information an attacker has on the targeted machine learning model. In this respect, adversarial attacks are divided into black-box and white-box attacks. •	Black-box attacks are practical settings where the attacker has limited information and access to the target ML model ~\cite{lei2018discrete}. The attacker’s capability is the same as a regular user and can only perform attacks given the allowed functions. The attacker also has no knowledge about the model and data used behind the service. In order to target the model, an attacker must probe it by repeatedly providing it with various inputs and evaluating its response until an adversarial vulnerability is discovered. On the other hand, White-box attacks usually assume complete knowledge and full transparency of the target model/data. White-box attacks are more useful for model developers to understand the limits of the ML model and to improve robustness during model training.

We randomly selected 300 instances each of Spam and Benign SMS from the test data to check the robustness of the model against the adversarial attacks. We then paraphrased the instances in 2 fold. In the first fold, we use a commercial tool Quillbot\footnote{https://quillbot.com/}. In the second phase, we manually check each of SMS instance paraphrase by Quillbot to make sure top 500 spam keywords (free, special offer, now, WIN, etc) in each SMS message are paraphrased and that the overall meaning/ semantic of the message is not lost. We then evaluated the model with the unaltered selected instances and the paraphrased sentences. As expected, the accuracy of the model on benign instances remains unchanged (100\%) whereas the accuracy of the spam instances drops significantly from 78\% to 36\%. Results of spam and benign instances before and after paraphrasing is given in Table 4.

\begin{table}
\begin{center}
\caption{Performance of Classifiers on Consolidated Dataset (cf. Table~\ref{tab:dataset} \textcolor{red}{What is consolidated dataset? Does Table~\ref{tab:dataset} enumerate this dataset?}.}
\newcolumntype{a}{>{\columncolor{red!50}}c}
\newcolumntype{b}{>{\columncolor{green!50}}c}
\begin{tabular}{ c | c | b | >{\columncolor{yellow!50}} c | a | a}
 \hline
 \emph{Feature Model} & \emph{Classifier} & \emph{Precision}&\emph{Recall} &\emph{F1 Score} &\emph{Accuracy}\\ [0.25ex]
 \hline\hline
  \multirow{ 3}{*}{BoW} & TCSVM & 0.96 & 0.87 &  0.91 & 0.96 \\
  & OCSVM & 0.72 & 0.70 & 0.71 & 0.82\\
  & PU & 0.98 & 0.93 & 0.95 & 0.96 \\
  \hline
  \multirow{ 3}{*}{Bigram} & TCSVM & 1.00 & 0.46 & 0.63 & 0.85 \\
  & OCSVM & 0.13 & 0.30 & 0.18 & 0.15\\
  & PU & 0.99 & 0.89 & 0.94 & 0.94 \\
  \hline
  \multirow{ 3}{*}{Trigram} & TCSVM & 1.00 & 0.36 & 0.53 & 0.84 \\
  & OCSVM & 0.21 & 0.55 & 0.30 & 0.18\\
  & PU & 1.00 & 0.86 & 0.92 & 0.93 \\
  \hline
  \multirow{ 3}{*}{5-gram} & TCSVM & 1.00 & 0.23 & 0.37 & 0.81 \\
  & OCSVM & 0.27 & 0.81 & 0.41 & 0.26\\
  & PU & 1.00 & 0.82 & 0.90 & 0.91 \\
  \hline
  \multirow{ 3}{*}{\makecell{Word2Vec \\ (static)}} & TCSVM & 0.93 & 0.91 & 0.92 & 0.96 \\
  & OCSVM & 0.37 & 0.91 & 0.53 & 0.47\\
  & PU & 0.75 & 0.95 & 0.84 & 0.81 \\
  \hline
    \multirow{ 3}{*}{\makecell{Glove \\ (static)}} & TCSVM & 0.93 & 0.94 & 0.93 & 0.936 \\
  & OCSVM & 0.74 & 0.49 & 0.47 & 0.491\\
  & PU & 0.596 & 0.944 &  & 0.845 \\
  \hline
  \hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
\caption{Performance of Deep Learning/ Neural Network Classifiers on Consolidated Dataset \textcolor{red}{What is consolidated dataset? Does Table~\ref{tab:dataset} enumerate this dataset?}.}
\newcolumntype{a}{>{\columncolor{red!50}}c}
\newcolumntype{b}{>{\columncolor{green!50}}c}
\begin{tabular}{ c | a | b | >{\columncolor{yellow!50}} c | a }
 \hline
 \emph{Classifier} & \emph{Feature Model} &\emph{Accuracy}\\ [0.25ex]
 \hline\hline
 {BERT (Google)} ~\cite{devlin2018bert} & bert-base-uncased & 0.98 \\
\hline 
\multirow{2}{*}{FastText (Facebook)} ~\cite{bojanowski2017enriching} & BoW & 0.965 \\
& Bigram & 0.976 \\ 
 \hline
 {ELMo (AllenNLP)} ~\cite{ELMo} & ELMO & 0.9517 \\
\hline 
{XLNet (Google Brain)} ~\cite{yang2019xlnet} & WordEmbedding-Random & 0.9631 \\
% \hline
% {GPT2/3  (OpenAI)} ~\cite{radford2019language} & - & In-progress \\
\hline
{RoBERTa} ~\cite{liu2019roberta} & roberta-base & 0.9895 \\
\hline
{XLM-RoBERTa} ~\cite{conneau2019cross} & xlm-roberta-base & 0.9725 \\ 
\hline
{DistilBERT} ~\cite{sanh2019distilbert} & distilbert-base-uncased & 0.9702 \\
\hline
Dense Network & WordEmbedding-Random & 0.9782 \\
\hline
LSTM & WordEmbedding-Random & 0.9614 \\
\hline
BiLSTM & WordEmbedding-Random & 0.9585 \\
\hline
\multirow{2}{*}{CNN} & WordEmbedding-Random & 0.9628 \\
& WordEmbedding-Static(GloVe) & 0.9642 \\
\hline
\multirow{4}{*}{TCN} & WordEmbedding-Random & 0.9762 \\
& WordEmbedding-Static (Word2Vec) & 0.9784 \\
& WordEmbedding-Dynamic (Word2Vec) & 0.9791 \\
\hline
\multirow{3}{*}{Ensemble (CNN-BiGRU)} & WordEmbedding-Random & 0.9722 \\
& WordEmbedding-Static (Word2Vec) & 0.9763 \\
& WordEmbedding-Dynamic (Word2Vec) & 0.9768\\
  \hline
  \hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
\caption{Performance of Classifiers on Super Dataset. \textcolor{red}{What is Super dataset? Does Table~\ref{tab:dataset} enumerate this dataset?}.}
\newcolumntype{a}{>{\columncolor{red!50}}c}
\newcolumntype{b}{>{\columncolor{green!50}}c}
\begin{tabular}{ c | c | b | >{\columncolor{yellow!50}} c | a | a}
 \hline
 \emph{Feature Model} & \emph{Classifier} & \emph{Precision}&\emph{Recall} &\emph{F1 Score} &\emph{Accuracy}\\ [0.25ex]
 \hline\hline
  \multirow{ 3}{*}{BoW} & TCSVM & 0.979 & 0.954 & 0.966 & 0.981 \\
  & OCSVM & 0.502 & 0.375 & 0.43 & 0.856\\
  & PU & 0.999 & 0.997 & 0.998 & 0.998 \\
  \hline
  \multirow{ 3}{*}{Bigram} & TCSVM & 0.995 & 0.756 & 0.859 & 0.93 \\
  & OCSVM & 0.068 & 0.316 & 0.112 & 0.273\\
  & PU & 0.999 & 0.997 & 0.998 & 0.998 \\
  \hline
  \multirow{ 3}{*}{Trigram} & TCSVM & 1.00 & 0.419 & 0.591 & 0.835 \\
  & OCSVM & 0.124 & 0.831 & 0.216 & 0.129\\
  & PU & 0.999 & 0.997 & 0.998 & 0.998 \\
  \hline
  \multirow{ 3}{*}{5-gram} & TCSVM & 1.00 & 0.148 & 0.258 & 0.759 \\
  & OCSVM & 0.143 & 0.985 & 0.249 & 0.143\\
  & PU & 0.999 & 0.997 & 0.998 & 0.998 \\
  \hline
  \multirow{ 3}{*}{Word2Vec} & TCSVM & 0.97 & 0.96 & 0.986 & 0.980 \\
  & OCSVM & 0.17 & 0.91 & 0.29 & 0.341\\
  & PU & 0.956 & 0.974 & 0.962 & 0.963 \\
  \hline
  \multirow{ 3}{*}{GloVe} & TCSVM & 0.95 & 0.95 & 0.95 & 0.952 \\
  & OCSVM & 0.85 & 0.33 & 0.36 & 0.331\\
  & PU & 0.966 & 0.976 &  & \\
  \hline
  \hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\begin{center}
\caption{Performance of Deep Learning/ Neural Network Classifiers on Super Dataset. \textcolor{red}{What is Super dataset? Does Table~\ref{tab:dataset} enumerate this dataset?}.}
\newcolumntype{a}{>{\columncolor{red!50}}c}
\newcolumntype{b}{>{\columncolor{green!50}}c}
\begin{tabular}{ c | a | b | >{\columncolor{yellow!50}} c | a }
 \hline
 \emph{Classifier} & \emph{Feature Model} &\emph{Accuracy}\\ [0.25ex]
 \hline\hline
 {BERT (Google)} ~\cite{devlin2018bert} & bert-base-uncased & 0.979 \\
\hline 
\multirow{2}{*}{FastText (Facebook)} ~\cite{bojanowski2017enriching} & BoW & 0.914 \\
& Bigram & 0.921 \\ 
 \hline
 {ELMo (AllenNLP)} ~\cite{ELMo} & ELMO & 0.983 \\
\hline
{RoBERTa} ~\cite{liu2019roberta}  & roberta-base & 0.975 \\
\hline
{XLM-RoBERTa} ~\cite{conneau2019cross}  & xlm-roberta-base & 0.971 \\ 
\hline
{DistilBERT} ~\cite{sanh2019distilbert} & distilbert-base-uncased & 0.98 \\
\hline
Dense Network & WordEmbedding-Random & 0.981 \\
\hline
LSTM & WordEmbedding-Random & 0.975 \\
\hline
BiLSTM & WordEmbedding-Random & 0.977 \\
\hline
\multirow{2}{*}{CNN} & WordEmbedding-Random & 0.978 \\
& WordEmbedding-Static(GloVe) & 0.979 \\
\hline
\multirow{4}{*}{TCN} & WordEmbedding-Random & 0.972 \\
& WordEmbedding-Static (Word2Vec) & 0.975 \\
& WordEmbedding-Dynamic (Word2Vec) & 0.974 \\
\hline
\multirow{3}{*}{Ensemble (CNN-BiGRU)} & WordEmbedding-Random & 0.979 \\
& WordEmbedding-Static (Word2Vec) & 0.983 \\
& WordEmbedding-Dynamic (Word2Vec) & 0.976\\
  \hline
  \hline
\end{tabular}
\end{center}
\end{table}

% \begin{table}
% \begin{center}
% \caption{Performance of Deep Learning Classifiers}
% \newcolumntype{a}{>{\columncolor{red!50}}c}
% \newcolumntype{b}{>{\columncolor{green!50}}c}
% \begin{tabular}{ c | c | b | >{\columncolor{yellow!50}} c | a }
%  \hline
%  \emph{Classifier} & \emph{Feature Model} & \emph{Precision}&\emph{Recall} &\emph{Accuracy}\\ [0.25ex]
%  \hline\hline
%  {BERT} & - & 0.98 & 0.98 & 0.98 \\
% \hline 
% Dense Network & - & - & - & 0.9642 \\
% \hline
% \multirow{4}{*}{TCN} & BoW & - & - & - \\
% & WordEmbedding-Random & - & - & 0.9762 \\
% & WordEmbedding-Static (Word2Vec) & - & - & 0.9784 \\
% & WordEmbedding-Dynamic (Word2Vec) & - & - & 0.9791 \\
% \hline
% \multirow{4}{*}{Ensemble (CNN-BiGRU)} & BoW & - & - & - \\
% & WordEmbedding-Random & - & - & 0.9722 \\
% & WordEmbedding-Static (Word2Vec) & - & - & 0.9763 \\
% & WordEmbedding-Dynamic (Word2Vec) & - & - & 0.9768\\
% \hline
% LSTM & - & - & - & - \\
% \hline
% Bi-LSTM & - & - & - & - \\ 
%   \hline
%   \hline
% \end{tabular}
% \end{center}
% \end{table}

\begin{table}
\caption{Performance of Classifiers After Paraphrasing Spam Messages (Paraphrasing Attack). \textcolor{red}{Which dataset was used in this attack?}}
\newcolumntype{a}{>{\columncolor{red!50}}c}
\newcolumntype{b}{>{\columncolor{green!50}}c}
\begin{tabular}{ c | c | b | b | b | a | a | a}
 \hline

 \emph{Feature Model} & \emph{Classifier} & \multicolumn{3}{c}{\emph{Before Paraphrasing}} & \multicolumn{3}{c}{\emph{After Paraphrasing}}\\
   & & Precision & Recall & Accuracy
   & Precision & Recall & Accuracy  \\
 \hline\hline

  \multirow{ 3}{*}{BoW} & TCSVM & 1.00 & 0.86 & 0.86 & 1.00 & 0.58 & 0.58 \\
  & OCSVM & 1.0 & 0.80 & 0.80 & 1.00 & 0.68 & 0.68\\
  & PU & 1.00 & 0.88 & 0.88 & 1.00 & 0.7 & 0.7 \\
  \hline
  \multirow{ 3}{*}{Bigram} & TCSVM & 1.00 & 0.62 & 0.62 & 1.00 & 0.06 & 0.06\\
  & OCSVM & 1.0 & 0.48 & 0.48 & 1.00 & 0.26 & 0.26\\
  & PU & 1.0 & 0.76 & 0.76 & 1.0 & 0.2 & 0.2\\
  & FastText & 0.98 & 0.98 & NA & 0.78 & 0.78 & NA\\
  \hline
  \multirow{ 3}{*}{Trigram} & TCSVM & 1.00 & 0.44 & 0.44 & 1.00 & 0.04 & 0.04 \\
  & OCSVM & 1.0 & 0.58 & 0.58 & 1.0 & 0.72 & 0.72\\
  & PU & 1.0 & 0.38 & 0.38 & 1.0 & NA & NA\\
  & FastText & 0.98 & 0.98 & NA & 0.78 & 0.78 & NA\\
  \hline
  \multirow{ 3}{*}{5-gram} & TCSVM & 1.00 & 0.38 & 0.38 & 1.00 & 0.00 & 0.00\\
  & OCSVM & 1.0 & 0.78 & 0.78 & 1.0 & 0.96 & 0.96\\
  & PU & 1.0 & 0.36 & 0.36 & 1.0 & 0.04 & 0.04\\
  & FastText & 0.98 & 0.98 & NA & 0.78 & 0.78 & NA\\
  \hline
  \multirow{ 3}{*}{Word2Vec} & TCSVM & 1.00 & 0.9 & 0.9 & 1.00 & 0.82 & 0.82\\
  & OCSVM & 1.0 & 0.68 & 0.68 & 1.0 & 0.68 & 0.68\\
  & PU & 1.0 & 0.96 & 0.96 & 1.0 & 0.98 & 0.98\\
  \hline
  \hline
\end{tabular}
\end{table}

\begin{table}
\begin{center}
\caption{Robustness/ Adversarial Evaluation of ML Classifiers on Super Dataset. \textcolor{red}{What is consolidated dataset? Does Table~\ref{tab:dataset} enumerate this dataset?}.}
\newcolumntype{a}{>{\columncolor{red!50}}c}
\newcolumntype{b}{>{\columncolor{green!50}}c}
\tabcolsep=0.15cm
\begin{tabular}{ c | c | b | a | a | a | a | a | a}
 \hline
 \emph{Feature Model} & \emph{Classifier} & \emph{Actual}&\emph{Paraphrasing} &\emph{EDA} &\emph{Homograph} &\emph{Spacing} &\emph{Charswap} &\emph{Hybrid}\\ [0.25ex]
 \hline\hline
  \multirow{ 3}{*}{BoW} & TCSVM & 0.809 & 0.511 & 0.791 & - & \textbf{0.284} & 0.356 & 0.298\\
  & OCSVM & 0.658 & 0.226 & 0.622 & 0.636 & \textbf{0.111} & 0.19 & \textbf{0.111}\\
  & PU & 0.836 & 0.622 & 0.818 & 0.822 & \textbf{0.32} & 0.427 & 0.329\\
  \hline
  \multirow{ 3}{*}{Bigram} & TCSVM & 0.480 & 0.107 & 0.444 & - & \textbf{0.102} & 0.058 & 0.102\\
  & OCSVM & 0.408 & 0.267 & 0.40 & \textbf{0.351} & \textbf{0.351} & 0.658 & 0.356\\
  & PU & 0.604 & 0.209 & 0.529 & 0.564 & 0.133 & \textbf{0.067} & 0.129\\
  \hline
  \multirow{ 3}{*}{Trigram} & TCSVM & 0.289 & 0.013 & 0.200 & 0.253 & 0.018 & \textbf{0.0} & 0.018\\
  & OCSVM & 0.662 & 0.804 & 0.627 & \textbf{0.64} & 0.764 & 0.964 & 0.769\\
  & PU & 0.338 & 0.036 & 0.236 & 0.298 & 0.022 & \textbf{0.0} & 0.022\\
  \hline
  \multirow{ 3}{*}{5-gram} & TCSVM & 0.200 & 0.000 & 0.089 & 0.178 & 0.009 & \textbf{0.0} & 0.009\\
  & OCSVM** & 0.751 & 0.986 & 0.786 & \textbf{0.733} & 0.951 & 1.00 & 0.951\\
  & PU & 0.204 & \textbf{0.0} & 0.062 & 0.156 & 0.004 & \textbf{0.0} & 0.004\\
  \hline
  \multirow{ 3}{*}{Word2Vec} & TCSVM & 0.831 & 0.76 & 0.831 & 0.333 & \textbf{0.116} & 0.396 & 0.173\\
  & OCSVM & 0.875 & 0.889 & 0.898 & 0.744 & 0.853 & \textbf{0.661} & 0.907\\
  & PU & 0.902 & 0.898 & 0.876 & 0.592 & 0.28 & \textbf{0.0} & 0.373\\
  \hline
  \multirow{ 3}{*}{GloVe} & TCSVM & 0.796 & 0.698 & 0.782 & 0.72 & 0.022 & 0.4 & 0.071\\
  & OCSVM & 0.916 & 0.942 & 0.928 & - & 0.347 & 0.671 & 0.547\\
  & PU & 0.858 & 0.88 & 0.8444 & 0.547 & 0.08 & 0.529 & 0.133 \\
  \hline
  \hline
\end{tabular}
\end{center}
\end{table}

**Further experimentation shows that OCSVM classify ham messages with insufficient accuracy... 

\begin{table}
\begin{center}
\caption{Robustness/ Adversarial Evaluation of Deep Learning/ Neural Network Classifiers on Super Dataset. \textcolor{red}{What is consolidated dataset? Does Table~\ref{tab:dataset} enumerate this dataset?}.}
\newcolumntype{a}{>{\columncolor{red!50}}c}
\newcolumntype{b}{>{\columncolor{green!50}}c}

\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}
\tabcolsep=0.15cm

\begin{tabular}{ c | c | b | a | a | a | a | a | a}
 \hline
 \emph{Classifier} & \emph{Feature Model} & \emph{Actual}&\emph{Para} &\emph{EDA} &\emph{Homograph} &\emph{Spacing} &\emph{Charswap} &\emph{Hybrid}\\ [0.1ex]
 \hline\hline
 {BERT} & bert-base-uncased & 0.898 & 0.778 & 0.884 & 0.684 & \textbf{0.249} & 0.698 & 0.4 \\
\hline 
\multirow{2}{*}{FastText} & BoW & 0.871 & 0.582 & 0.849 & 0.613 & \textbf{0.378} &  0.542 & 0.569\\
& Bigram & 0.893 & 0.591 & 0.902 & 0.649 & \textbf{0.44} & 0.653 & 0.658\\ 
 \hline
 {ELMo} & ELMO & 0.893 & 0.777 & 0.879 & 0.839 & \textbf{0.446} & 0.821 & 0.554 \\
% \hline 
% {XLNet} & xlnet-base-cased & - & - & - & - & - & - & - \\
% \hline
% {GPT2/3  (OpenAI)} ~\cite{radford2019language} & - & In-progress \\
\hline
{RoBERTa}  & roberta-base & 0.929 & 0.836 & 0.924 & - & \textbf{0.516} & 0.893 & 0.813 \\
\hline
{XLM-RoBERTa} & xlm-roberta-base & 0.902 & 0.782 & 0.898 & 0.911 & \textbf{0.342} & 0.831 & 0.542 \\ 
\hline
{DistilBERT} & distilbert-base-uncased & 0.951 & 0.836 & 0.929 & 0.787 & \textbf{0.431} & 0.76 & 0.631 \\
\hline
Dense Network & WE-Random & 0.769 & 0.587 & 0.751 & 0.475 & \textbf{0.124} & 0.618 & 0.151 \\
\hline
LSTM & WE-Random & 0.7511 & 0.533 & 0.724 & 0.422 & \textbf{0.098} & 0.560 & 0.147 \\
\hline
BiLSTM & WE-Random & 0.702 & 0.484 & 0.68 & 0.287 & \textbf{0.084} & 0.449 & 0.111 \\
\hline
\multirow{2}{*}{CNN} & WE-Random & 0.742 & 0.507 & 0.702 & 0.341 & \textbf{0.076} & 0.507 & 0.124 \\
& WE-Static(GloVe) & 0.787 & 0.547 & 0.773 & 0.422 & \textbf{0.071} & 0.569 & 0.111 \\
\hline
\multirow{4}{*}{TCN} & WE-Random & 0.809 & 0.684 & 0.804 & 0.609 & \textbf{0.24} & 0.551 & 0.178 \\
& WE-Static (Word2Vec) & 0.831 & 0.738 & 0.822 & 0.72 & 0.151 & 0.769 & \textbf{0.124} \\
& WE-Dynamic (Word2Vec) & 0.911 & 0.804 & 0.907 & 0.876 & \textbf{0.422} & 0.889 & 0.436 \\
\hline
\multirow{3}{*}{\makecell{Ensemble \\ (CNN-BiGRU)}} & WE-Random & 0.791 & 0.68 & 0.791 & 0.586 & 0.124 & 0.649 & \textbf{0.093} \\
& WE-Static (Word2Vec) & 0.876 & 0.858 & 0.858 & 0.84 & \textbf{0.124} & 0.876 & 0.16 \\
& WE-Dynamic (Word2Vec) & 0.849 \ & 0.791 & 0.858 & 0.653 & 0.276 & 0.698 & \textbf{0.244}\\
  \hline
  \hline
\end{tabular}
\end{center}
\end{table} 

\subsubsection{One-class SVM}
One-class SVM is an unsupervised algorithm that learns a decision function for novelty detection: classifying new data as similar or different to the training set [ref]. The one-class algorithms are based on recognition since their aim is to recognize data from a particular class, and reject data from all other classes. This is accomplished by creating a boundary that encompasses all the data belonging to the target class within itself, so when a new sample arrives the algorithm only has to check whether it lies within the boundary or outside and accordingly classify the sample as belonging to the target class or the outlier.

\textbf{Pre-processing and Normalization} During the pre-processing stage, we considered spam SMS as our training class and replaced the spam label with 1 and all other labels (ham, nil) with -1 because one-class classification model prediction will be 1 or -1 (1 is the target class and -1 is the outlier). Accordingly, we divided the SMS corpus into training set (spam instances) and test set (comprise of benign and unlabeled instances). Further we cleaned (removed stop words and special characters, truncated word to its base form using lemmatization) and tokenized the text using the spaCy [footnote] tool in python.

\textbf{Feature Extraction, Embedding and Vectorization}.  Next we converted the tokenized text (list of words) to an actual vector using SciKit Learn's HashingVectorizer. The HashingVectorizer method converted the collection of text to a matrix of token occurrences. The advantage of using the HashingVectorizer over the Countvectorizer is that it does not store the resulting vocabulary (i.e. the unique tokens). The benefit of not storing the vocabulary (dictionary of tokens) is two folded. First, this is very efficient for a large dataset. Holding a 300M token vocabulary in memory could be a challenge in certain computing environments as these are essentially strings. It demands more memory compared to their integer counterparts. By not having to store the vocabulary, the resulting HashingVectorizer object when saved, would be much smaller and thus faster to load back into memory when needed. We extracted the same set of syntactic and semantic features discussed in Sec 6.2.1. 

\textbf{Model Building and Evaluation}.  Finally, we trained the one-class SVM model over the spam instances to develop a model for spam detection. We then evaluated the model performance on the test data; performance details (Precision, recall and accuracy) of the model is presented in 3. 

\textbf{Adversarial Evaluation of Model Performances (Exploiting/ Evading the Model)}. After evaluating the model on test set, we checked the robustness of the one-class SVM by paraphrasing randomly selected 50 instances each of Spam and Benign using the same approached as discussed in the subsection??. Results of spam and benign instances before and after paraphrasing is given in Table 4.

For Adversarial example cite below somewhere

OpenAttack (https://github.com/thunlp/OpenAttack) and papers
textAttack
textbug
deepbug
textfooler
TFAadjusted/ GeneticAttack

\subsubsection{PU Learning}
PU learning is a semi-supervised binary classification method that recovers labels from unknown cases in the data. It does this by learning from the positive cases in the data and applying what it has learned to relabel the unknown cases. This approach provides benefits to any machine learning problem that requires binary classification on unreliable data, regardless of the domain.
We implemented the PU learning to perform classification on our SMS corpus since we are cursed with the similar problem of imbalanced and unreliable dataset. Our dataset (ref table 2) have few positive labels (\% of positive labels), 000\% unreliable labels since more than 64,000 (mention accurate no) out of 73,000 (mention accurate no) are labeled using Google spam detection tool and a large no (\%) of benign and unlabeled SMS instances. Details of the dataset used for PU learning is presented in Table 2.

\textbf{Pre-processing and Normalization}. First, we balanced the both the major (unlabeled) and minor (positive) class in the data evenly to have 27,103 of class 0 and 27,103 of class 1 by down sampling the majority class to match the minority class [ref]. Next we perform text pre-processing (or cleaning) as discussed in subsection.

\textbf{Feature Extraction, Embedding and Vectorization}. We extracted the same set of syntactic and semantic features discussed in section 6.2.1.

\textbf{Model Building and Evaluation}. We first started developing a model by training a standard random forest classifier and then compared the result to the original labels. As evident from Table 3, the standard random forest did not do very well for predicting the hidden positives in unlabeled. Only 50\% recall, meaning it did not recover any of the hidden positive classes. Therefore, we extended this further by jumping into PU bagging. The PU bagging is an approach for training many ensemble classifiers in parallel. It is basically an ensemble of ensembles. With each ensemble, the classes are balanced to the size of the positive class. We received quite good results for PU bagging approach with random forest (results presented in table 3). It is clear that PU Bagging is doing significantly better.

\textbf{PU Bagging}. First Randomly sample all positives and a subset of unlabeled data.
Next, Build a classifier with this bootstrapped dataset (using positive as 1 and unknown as 0) and then predict the classes of unknowns that were not sampled in training (known as Out-of-bag samples). Repeat many times and get the OOB average scores. PUBagging is quicker than normal ensemble methods (especially with tree based algorithms) as it makes use of parallelization and provides better accuracy for Tree based algorithms (Two step approach). PUBagging provides the best results with SVM's, however it it takes incredibly long to train.


\subsubsection{Preliminary Analysis}
\textbf{Key Takeaway} From Table 3 and Table 4, it can be concluded that the context play a vital role towards classification and outcome of the spam detection as the accuracy of the classifiers decreases significantly when the no of tokens (n-grams) increase. Therefore, we decided to apply context-free word embedding like Word2Vec and FastText which maps similar words to same coordinates. This is one potential way to counter the paraphrasing attacks due to its ability to map similar words to same coordinates. 

\section{Evaluation/ Assessment}
This work/ section presents a number of statistics, studies and baseline results for several machine learning and deep learning methods.The performance and robustness of the aforementioned classifiers were assessed following two stages. 

Performance evaluation: In first stage, the classifiers were evaluated on test and train split..... 

Robustness. In second stage, the robustness of the aforementioned classifiers were assessed by designing a no of adversarial attacks....

==> files/rwork.tex <==
SMS spam detection is a very important job for people who use cell phones. It can lessen the irritation caused by the intrusive marketing performed using this platform. It can also make the user experience safer by blocking messages that might be dangerous. In that sense, researchers have come up with different ways to tell if a text message is spam. 

A lot of information about fraud schemes in telephony network have been discussed in the academic literature and can be found in white papers by companies selling fraud detection systems~\cite{subexfraud}~\cite{Transfraud}. However, most of the papers focus on voice scam~\cite{sahin2017sok} especially spam in the Voice over IP (VoIP) domain and PSTN telephony network. The whitepapers published by industrial sector often present an incomplete view of the threat landscape because of the possible commercial interests whereas the academic literature handle only part of the problem or try to reduce the problem into a single dimension such as actors (fraudster or victim) ~\cite{Wikifraud}, attack methodology or attack motivation ~\cite{becker2010fraud}. However, the scam ecosystem is too complex to be explained with a binary classification. ~\cite{anderson2020security} studies the telecom system security, covering many fraud related topics. It concludes that information on phone fraud is scattered and no single resource brings everything together. Existing surveys ~\cite{becker2010fraud} address fraud detection, but do not try to systematize the fraud itself.
In ~\cite{gupta2015phoneypot}, ~\cite{balduzzi2016mobipot} authors analyze data from phone honeypots uncovering several fraud schemes affecting end users. ~\cite{tu2016sok} analyzes the voice spam ecosystem and evaluates existing solutions. However, none of these resources provide a comprehensive view of the SMS scam ecosystem.

Scammers use a variety of methods to extort money from innocent people. Stajano and Wilson ~\cite{stajano2011understanding} investigated a variety of fraud schemes and demonstrated the value of security engineering activities. Buchanan and Grant ~\cite{buchanan2001investigating} offered a brief description of Nigerian scam schemes, emphasizing that the growth of the Internet has aided the proliferation of cyber-crime. Coomer ~\cite{Patent655} recently received a patent for a technology that uses phone number analysis to detect fraud and spam emails. One of the challenge in spam detection is the dynamic behavior of scammers. They always try to find a way to deceive the spam filters using different adversarial attacks.

In order to disrupt the anticipated behavior of a prediction model, adversarial attack strategies usually include carefully manipulating the nature of the input data ~\cite{laskov2010machine}. The research of adversarial environments first gained traction over a decade ago, when the weaknesses of spam filters exposed to this form of manipulation were discovered ~\cite{biggio2018wild}. Many adversarial attacks and defenses have been documented since then in a number of applications, including online abusive comments and profanity detection ~\cite{rodriguez2018shielding,rojas2017obstructing,hosseini2017deceiving,sood2012profanity}, medical picture classification ~\cite{finlayson2019adversarial}, and object recognition in computer vision ~\cite{akhtar2018threat,hosseini2017google}, to name a few.

Attacks on text classification activities are typically carried out by altering characteristics or manipulating the text sequence's content ~\cite{rojas2017obstructing}. Several approaches have been identified in the field of adversarial operations against spam filters in particular ~\cite{kuchipudi2020adversarial,imam2019survey}: poisoning, injection of good words, obfuscation of spam words, label changes, and synonym replacement etc.

